Conway's drum quilts

A `transplantable pair' is a pair of glueing diagrams that can be used to create pairs of plane domains that are isospectral for the Laplace operator. We present a host of transplantable pairs worked out by John Conway using his theory of quilts

==> quilt_dot_bib <==
@article {bcds:drum,
    AUTHOR = {Buser, Peter and Conway, John and Doyle, Peter and Semmler,
              Klaus-Dieter},
     TITLE = {Some planar isospectral domains},
   JOURNAL = {Internat. Math. Res. Notices},
      YEAR = {1994},
    VOLUME = {9},
eprint={arXiv:1005.1839v1 [math.DG]},
note={\url{http://arxiv.org/abs/1005.1839v1}}
}


@book {conway:sensual,
    AUTHOR = {Conway, John H.},
     TITLE = {The sensual (quadratic) form},
    SERIES = {Carus Mathematical Monographs},
    VOLUME = {26},
      NOTE = {With the assistance of Francis Y. C. Fung},
 PUBLISHER = {Mathematical Association of America},
      YEAR = {1997}
}


@incollection {conway:notation,
    AUTHOR = {Conway, J. H.},
     TITLE = {The orbifold notation for surface groups},
 BOOKTITLE = {Groups, combinatorics \& geometry ({D}urham, 1990)},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {165},
     PAGES = {438--447},
 PUBLISHER = {Cambridge},
      YEAR = {1992}
}

@book{conway:things,
author={Conway, John. H. and Burgiel, Heidi and Goodman-Strauss, Chaim},
title={The Symmetries of Things},
publisher={Taylor and Francis},
year={2008}
}

@incollection {bb:selberg,
   AUTHOR = {B{\'e}rard-Bergery, Lionel},
    TITLE = {Laplacien et g\'eod\'esiques ferm\'ees sur les formes d'espace
             hyperbolique compactes},
 BOOKTITLE = {S\'eminaire Bourbaki, 24\`eme ann\'ee (1971/1972), Exp. No.
             406},
    PAGES = {107--122. Lecture Notes in Math., Vol. 317},
 PUBLISHER = {Springer},
  ADDRESS = {Berlin},
     YEAR = {1973},
  MRCLASS = {53C20 (58G99)},
 MRNUMBER = {MR0420504 (54 \#8518)},
MRREVIEWER = {Midori Goto},
ZBL={0261.53034}
}

@book {buser:book,
   AUTHOR = {Buser, Peter},
    TITLE = {Geometry and spectra of compact {R}iemann surfaces},
   SERIES = {Progress in Mathematics},
   VOLUME = {106},
 PUBLISHER = {Birkh\"auser Boston Inc.},
  ADDRESS = {Boston, MA},
     YEAR = {1992},
    PAGES = {xiv+454},
     ISBN = {0-8176-3406-1},
  MRCLASS = {58G25 (30F99)},
 MRNUMBER = {MR1183224 (93g:58149)},
MRREVIEWER = {Robert Brooks},
ZBL={0770.53001}
}


@book {chavel:eigen,
   AUTHOR = {Chavel, Isaac},
    TITLE = {Eigenvalues in {R}iemannian geometry},
   SERIES = {Pure and Applied Mathematics},
   VOLUME = {115},
     NOTE = {Including a chapter by Burton Randol,
             With an appendix by Jozef Dodziuk},
 PUBLISHER = {Academic Press Inc.},
  ADDRESS = {Orlando, FL},
     YEAR = {1984},
    PAGES = {xiv+362},
     ISBN = {0-12-170640-0},
  MRCLASS = {58G25 (35P99 53C20)},
 MRNUMBER = {MR768584 (86g:58140)},
MRREVIEWER = {G{\'e}rard Besson},
ZBL={0551.53001}
}

@incollection {conway:orbifold,
   AUTHOR = {Conway, J. H.},
    TITLE = {The orbifold notation for surface groups},
 BOOKTITLE = {Groups, combinatorics \& geometry (Durham, 1990)},
   SERIES = {London Math. Soc. Lecture Note Ser.},
   VOLUME = {165},
    PAGES = {438--447},
 PUBLISHER = {Cambridge Univ. Press},
  ADDRESS = {Cambridge},
     YEAR = {1992},
  MRCLASS = {57M50 (20F32 57M60)},
 MRNUMBER = {MR1200280 (94a:57025)},
MRREVIEWER = {Denis Sjerve},
ZBL={0835.20048}
}

@article{selberg:harmonic,
AUTHOR={Atle Selberg},
TITLE={Harmonic analysis and discontinuous groups in weakly symmetric {R}iemannian spaces with applications to {D}irichlet series},
JOURNAL={J. Indian Math. Soc. B},
VOLUME={20},
YEAR={1956},
PAGES={47--87},
NOTE={Reprinted in \cite{selberg:harmonic1}}
}

@incollection{selberg:harmonic1,
        author =        "Atle Selberg",
        title =         "Harmonic analysis and discontinuous groups in weakly symmetric {R}iemannian spaces with applications to {D}irichlet series",
        pages =         "423--463",
        booktitle =     "Collected Papers, vol. 1",
        publisher =     "Springer",
        year =          "1989"
}



@article {doylerossetti:cosmic,
   AUTHOR = {Doyle, Peter G. and Rossetti, Juan Pablo},
    TITLE = {Tetra and {D}idi, the cosmic spectral twins},
  JOURNAL = {Geom. Topol.},
 FJOURNAL = {Geometry and Topology},
   VOLUME = {8},
     YEAR = {2004},
    PAGES = {1227--1242 (electronic)},
     ISSN = {1465-3060},
  MRCLASS = {58J53 (11F72 57M50 57N15)},
 MRNUMBER = {MR2087082 (2005j:58046)},
MRREVIEWER = {Dorothee Schueth},
ZBL={1091.58021}
}

@article {gangolli:selberg,
   AUTHOR = {Gangolli, Ramesh},
    TITLE = {The length spectra of some compact manifolds of negative
             curvature},
  JOURNAL = {J. Differential Geom.},
 FJOURNAL = {Journal of Differential Geometry},
   VOLUME = {12},
     YEAR = {1977},
   NUMBER = {3},
    PAGES = {403--424},
     ISSN = {0022-040X},
  MRCLASS = {58G99 (10D15)},
 MRNUMBER = {MR0650997 (58 \#31311)},
ZBL={0365.53016}
}

@article {huber:selbergI,
   AUTHOR = {Huber, Heinz},
    TITLE = {Zur analytischen {T}heorie hyperbolischen {R}aumformen und
             {B}ewegungsgruppen},
  JOURNAL = {Math. Ann.},
 FJOURNAL = {Mathematische Annalen},
   VOLUME = {138},
     YEAR = {1959},
    PAGES = {1--26},
     ISSN = {0025-5831},
  MRCLASS = {30.00},
 MRNUMBER = {MR0109212 (22 \#99)},
MRREVIEWER = {J. Lehner},
ZBL={0089.06101}
}

@article {phillipssarnak:PGT,
   AUTHOR = {Phillips, Ralph and Sarnak, Peter},
    TITLE = {Geodesics in homology classes},
  JOURNAL = {Duke Math. J.},
 FJOURNAL = {Duke Mathematical Journal},
   VOLUME = {55},
     YEAR = {1987},
   NUMBER = {2},
    PAGES = {287--297},
     ISSN = {0012-7094},
    CODEN = {DUMJAO},
  MRCLASS = {58F17 (11F72 58F18)},
 MRNUMBER = {MR894581 (88g:58151)},
MRREVIEWER = {Midori Goto},
ZBL={0642.53050}
}

@article {sunada:method,
   AUTHOR = {Sunada, Toshikazu},
    TITLE = {Riemannian coverings and isospectral manifolds},
  JOURNAL = {Ann. of Math. (2)},
 FJOURNAL = {Annals of Mathematics. Second Series},
   VOLUME = {121},
     YEAR = {1985},
   NUMBER = {1},
    PAGES = {169--186},
     ISSN = {0003-486X},
    CODEN = {ANMAAH},
  MRCLASS = {58G25 (11F72 53C20 57M99)},
 MRNUMBER = {MR782558 (86h:58141)},
MRREVIEWER = {Scott Wolpert},
ZBL={0585.58047}
}

@article {vigneras:isospectral,
   AUTHOR = {Vign{\'e}ras, Marie-France},
    TITLE = {Vari\'et\'es riemanniennes isospectrales et non
             isom\'etriques},
  JOURNAL = {Ann. of Math. (2)},
 FJOURNAL = {Annals of Mathematics. Second Series},
   VOLUME = {112},
     YEAR = {1980},
   NUMBER = {1},
    PAGES = {21--32},
     ISSN = {0003-486X},
    CODEN = {ANMAAH},
  MRCLASS = {58G25 (10J25 12A70)},
 MRNUMBER = {MR584073 (82b:58102)},
MRREVIEWER = {P. Wintgen},
ZBL={0445.53026}
}

@misc{drydenfinite,
title = {{Isospectral Finiteness of Hyperbolic Orbisurfaces}},
author = {Emily B. Dryden},
year="2004",
eprint = {arXiv:math.SP/0411290}}

@misc{drydenstrohmaier,
title = {{Huber's theorem for hyperbolic orbisurfaces}},
author = {Emily B. Dryden and Alexander Strohmaier},
year="2005",
eprint = {arXiv:math.SP/0504571}}

@misc{doylerossetti:verso,
title = {{Isospectral hyperbolic surfaces have matching geodesics}},
author = {Peter G. Doyle and Juan Pablo Rossetti},
year="2008",
eprint = {arXiv:math/0605765v2 [math.DG]}}

@misc{drydenetal,
title="Asymptotic expansion of the heat kernel for orbifolds",
author="Emily B. Dryden and Carolyn S. Gordon and Sarah J. Greenwald",
year="2008"
}

@article {berard:repequiv,
    AUTHOR = {B{\'e}rard, Pierre},
     TITLE = {Transplantation et isospectralit\'e. {II}},
   JOURNAL = {J. London Math. Soc. (2)},
  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {48},
      YEAR = {1993},
    NUMBER = {3},
     PAGES = {565--576},
      ISSN = {0024-6107},
     CODEN = {JLMSAK},
   MRCLASS = {58G25 (53C20)},
  MRNUMBER = {MR1241789 (95b:58153)},
MRREVIEWER = {Carolyn Gordon},
       DOI = {10.1112/jlms/s2-48.3.565},
       URL = {http://dx.doi.org/10.1112/jlms/s2-48.3.565},
}

@article {deturckgordon:selberg,
    AUTHOR = {DeTurck, Dennis M. and Gordon, Carolyn S.},
     TITLE = {Isospectral deformations. {II}. {T}race formulas, metrics, and
              potentials},
      NOTE = {With an appendix by Kyung Bai Lee},
   JOURNAL = {Comm. Pure Appl. Math.},
  FJOURNAL = {Communications on Pure and Applied Mathematics},
    VOLUME = {42},
      YEAR = {1989},
    NUMBER = {8},
     PAGES = {1067--1095},
      ISSN = {0010-3640},
     CODEN = {CPAMA},
   MRCLASS = {58G25 (53C20)},
  MRNUMBER = {MR1029118 (91e:58197)},
MRREVIEWER = {Klaus-Dieter Kirchberg},
       DOI = {10.1002/cpa.3160420803},
       URL = {http://dx.doi.org/10.1002/cpa.3160420803},
}

@Misc{stanhopeuribe:new,
  author = {Elizabeth Stanhope and Alejandro Uribe},
  howpublished      = 	 {Rumor},
  year = 2010
}

@article {wallach:stf,
    AUTHOR = {Wallach, Nolan R.},
     TITLE = {On the {S}elberg trace formula in the case of compact
              quotient},
   JOURNAL = {Bull. Amer. Math. Soc.},
  FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {82},
      YEAR = {1976},
    NUMBER = {2},
     PAGES = {171--195},
      ISSN = {0002-9904},
   MRCLASS = {22E45 (32N10 10D15)},
  MRNUMBER = {MR0404533 (53 \#8333)},
MRREVIEWER = {O. M. Fomenko},
}

@preamble{
   "\def\cprime{$'$} "
}
@book {gelfandetal,
    AUTHOR = {Gel{\cprime}fand, I. M. and Graev, M. I. and
              Pyatetskii-Shapiro, I. I.},
     TITLE = {Representation theory and automorphic functions},
    SERIES = {Generalized Functions},
    VOLUME = {6},
      NOTE = {Translated from the Russian by K. A. Hirsch,
              Reprint of the 1969 edition},
 PUBLISHER = {Academic Press Inc.},
   ADDRESS = {Boston, MA},
      YEAR = {1990},
     PAGES = {xviii+426},
      ISBN = {0-12-279506-7},
   MRCLASS = {11F70 (22E40 22E45 22E50 22E55)},
  MRNUMBER = {MR1071179 (91g:11052)},
}

@article{gordonWebbWolpert:drum,
        author =        "C. Gordon and D. Webb and S. Wolpert",
        title =         "One cannot hear the shape of a drum",
        journal =       "Bull. Amer. Math. Soc.",
        volume =        "27",
        year =          "1992",
        pages =         "134-138"
}


@article{ikeda:lens,
author="Akira Ikeda",
title="Lens spaces which are isospectral but not isometric",
journal="Annales Scientifiques de l'E. N. S.",
volume="13",
year="1980",
pages="303-315"
}

@incollection{ikeda:lensp,
    AUTHOR = {Akira Ikeda},
     TITLE = {Riemannian manifolds $p$-isospectral but not $(p+1)$-isospectral},
 BOOKTITLE = {Geometry of Manifolds},
 PUBLISHER = {Academic Press},
     PAGES = {383-417},
      YEAR = {1989}
}

@article {pesce:strong,
    AUTHOR = {Pesce, Hubert},
     TITLE = {Vari\'et\'es hyperboliques et elliptiques fortement
              isospectrales},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {134},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {363--391},
      ISSN = {0022-1236},
     CODEN = {JFUAAW},
   MRCLASS = {58G25 (53C20)},
  MRNUMBER = {1363805 (97a:58191)},
MRREVIEWER = {Carolyn Gordon},
       DOI = {10.1006/jfan.1995.1150},
       URL = {http://dx.doi.org/10.1006/jfan.1995.1150},
}

@article {schwartz:obtuse2,
    AUTHOR = {Schwartz, Richard Evan},
     TITLE = {Obtuse triangular billiards. {II}. {O}ne hundred degrees worth
              of periodic trajectories},
   JOURNAL = {Experiment. Math.},
  FJOURNAL = {Experimental Mathematics},
    VOLUME = {18},
      YEAR = {2009},
    NUMBER = {2},
     PAGES = {137--171},
      ISSN = {1058-6458},
   MRCLASS = {37D50 (37C25 37E15 37M99)},
  MRNUMBER = {2549685 (2010g:37060)},
MRREVIEWER = {Serge E. Troubetzkoy},
       URL = {http://projecteuclid.org/getRecord?id=euclid.em/1259158426},
}

@article {schwartz:obtuse1,
    AUTHOR = {Schwartz, Richard Evan},
     TITLE = {Obtuse triangular billiards. {I}. {N}ear the {$(2,3,6)$}
              triangle},
   JOURNAL = {Experiment. Math.},
  FJOURNAL = {Experimental Mathematics},
    VOLUME = {15},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {161--182},
      ISSN = {1058-6458},
   MRCLASS = {37D50 (37C25 37E15 37J10)},
  MRNUMBER = {2253003 (2007c:37034)},
MRREVIEWER = {Serge E. Troubetzkoy},
       URL = {http://projecteuclid.org/getRecord?id=euclid.em/1175789737},
}

@article {conwayhsu:quilts,
    AUTHOR = {Conway, John H. and Hsu, Tim},
     TITLE = {Quilts and {$T$}-systems},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {174},
      YEAR = {1995},
    NUMBER = {3},
     PAGES = {856--908},
      ISSN = {0021-8693},
     CODEN = {JALGA4},
   MRCLASS = {20F36 (57M05)},
  MRNUMBER = {1337175 (96m:20060)},
MRREVIEWER = {Geoffrey Mason},
       DOI = {10.1006/jabr.1995.1157},
       URL = {http://dx.doi.org/10.1006/jabr.1995.1157},
}

